Exact Moment Estimation of Stochastic Differential Dynamics

Moment estimation for stochastic differential equations (SDEs) is fundamental to the formal reasoning and verification of stochastic dynamical systems, yet remains challenging and is rarely available in closed form. In this paper, we study time-homogeneous SDEs with polynomial drift and diffusion, and investigate when their moments can be computed exactly. We formalize the notion of moment-solvable SDEs and propose a generic symbolic procedure that, for a given monomial, attempts to construct a finite linear ordinary differential equation (ODE) system governing its moment, thereby enabling exact computation. We introduce a syntactic class of pro-solvable SDEs, characterized by a block-triangular structure, and prove that all polynomial moments of any pro-solvable SDE admit such finite ODE representations. This class strictly generalizes linear SDEs and includes many nonlinear models. Experimental results demonstrate the effectiveness of our approach.

==> macros.tex <==

% Todonotes
\RequirePackage{todonotes}

\newcommand{\sfcomment}[1]{\todo[color=NavyBlue!30,size=\small,fancyline,author=Shenghua]{#1}\xspace}
\newcommand{\sfcommentinline}[1]{\todo[inline,color=NavyBlue!30,author=Shenghua]{#1}\xspace}
\newcommand{\atsf}{\colorbox{NavyBlue!30}{\textbf{@Shenghua}}}

\newcommand{\oomit}[1]{}

\newcommand{\myparagraph}[1]{\medskip\noindent{\bf #1.}}

\newcommand{\nzcomment}[1]{\todo[color=Orange!30,size=\small,fancyline,author=Naijun]{#1}\xspace}
\newcommand{\nzcommentinline}[1]{\todo[inline,color=Orange!30,author=Naijun]{#1}\xspace}
\newcommand{\atnz}{\colorbox{Orange!30}{\textbf{@Naijun}}}

\newcommand{\ajcomment}[1]{\todo[color=Green!30,size=\small,fancyline,author=anjie]{#1}\xspace}

%Colors
\definecolor{myred}{HTML}{e41a1c}
\definecolor{myblue}{HTML}{377eb8}
\definecolor{mygreen}{HTML}{4daf4a}
\definecolor{mygray}{gray}{0.6}
\definecolor{myorange}{HTML}{ffa510}
\newcommand{\green}[1]{\textcolor{mygreen}{#1}}
\newcommand{\red}[1]{\textcolor{myred}{#1}}
\newcommand{\blue}[1]{\textcolor{myblue}{#1}}
\newcommand{\violet}[1]{\textcolor{RedViolet}{#1}}
\newcommand{\orange}[1]{\textcolor{myorange}{#1}}
\newcommand{\gray}[1]{\textcolor{mygray}{#1}} 

% Real, Natural ...
\newcommand{\Reals}{\mathbb{R}\xspace}
\newcommand{\PosReals}{\mathbb{R}_{> 0}\xspace}
\newcommand{\NonNegReals}{\mathbb{R}_{\ge 0}\xspace}
\newcommand{\Realn}{\mathbb{R}^n\xspace}
\newcommand{\Nats}{\mathbb{N}\xspace}
\newcommand{\PosNats}{\mathbb{N}_{>0}\xspace}
\newcommand{\Ints}{\mathbb{Z}\xspace}

% Vectors
\newcommand{\ff}{\bm{f}\xspace}
\newcommand{\xx}{\bm{x}\xspace}
\newcommand{\yy}{\bm{y}\xspace}
\newcommand{\uu}{\bm{u}\xspace}
\newcommand{\fa}{\bm{a}\xspace}
\newcommand{\fb}{\bm{b}\xspace}
\newcommand{\xxi}{\bm{\xi}\xspace}
\newcommand{\RR}{\Reals}
\newcommand{\norm}[1]{\left\lvert#1\right\rvert}
\newcommand*{\trans}{\mathsf{T}}
\newcommand{\EE}{\mathbb{E}\xspace}

% \llangle for [[, \rragnel for ]]
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1[}\)}%
  \mathopen{\copy\@brx\kern-0.6\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1]}\)}%
  \mathclose{\copy\@brx\kern-0.6\wd\@brx\usebox{\@brx}}}
\makeatother


\newcommand{\qe}{\ensuremath{\mathtt{QE}}\xspace}
\newcommand{\fp}{\scriptsize{(\textsf{fp})}}
\newcommand{\mcheck}{\usym{1F5F8}}
\newcommand{\mtimes}{\scriptsize{\usym{2613}}}


%%%%    Standards    %%%%

\newcommand{\mydot}{\text{{\Large\textbf{.}}~}}
\DeclareMathOperator{\dif}{\,d\!}
\newcommand{\stag}[1]{{\tag*{\small{({#1})}}}}
\newcommand{\TAG}[1]{{\tag*{\small{[{#1}]}}}}
\newcommand*\from{\colon}
\newcommand{\supp}{\mathtt{supp}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%%%%    Shortcuts    %%%%

\newcommand{\minimize}{\mathtt{minimize}}
\newcommand{\subj}{\mathtt{subject~to}}


\newcommand{\tiff}{\textnormal{iff}\quad}
\newcommand{\qiff}{\ \quad\textnormal{iff}\quad\ }
\newcommand{\qqiff}{\qquad\textnormal{iff}\qquad}
\newcommand{\lqiff}{\textnormal{iff}\quad}
\newcommand{\lqqiff}{\textnormal{iff}\qquad}

\newcommand{\aand}{\ \ \textnormal{and}\ \ }
\newcommand{\qand}{\ \quad\textnormal{and}\quad\ }
\newcommand{\qqand}{\qquad\textnormal{and}\qquad}

\newcommand{\oor}{\ \ \textnormal{or}\ \ }
\newcommand{\qor}{\ \quad\textnormal{or}\quad\ }
\newcommand{\qqor}{\qquad\textnormal{or}\qquad}

\newcommand{\ffor}{\ \ \textnormal{for}\ \ }
\newcommand{\fforany}{\ \ \textnormal{for any}\ \ }
\newcommand{\qfor}{\ \quad\textnormal{for}\quad\ }
\newcommand{\qqfor}{\qquad\textnormal{for}\qquad}

\newcommand{\wwith}{\ \ \textnormal{with}\ \ }
\newcommand{\qwith}{\ \quad\textnormal{with}\quad\ }
\newcommand{\qqwith}{\qquad\textnormal{with}\qquad}

\newcommand{\qimplies}{\ \quad\textnormal{implies}\quad\ }
\newcommand{\qqimplies}{\qquad\textnormal{implies}\qquad}
\newcommand{\lqimplies}{\textnormal{implies}\quad}
\newcommand{\lqqimplies}{\textnormal{implies}\qquad}

\newcommand{\pprec}{\mathrel{{\prec}\hspace{-.5ex}{\prec}}}
\newcommand{\ppprec}{~{}\pprec{}~}
\newcommand{\npprec}{\centernot\pprec}

\newcommand{\ppreceq}{~{}\preceq{}~}
\newcommand{\ssucceq}{~{}\succeq{}~}
\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\define}{\defeq}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}
\newcommand{\mmapsto}{~{}\mapsto{}~}
\newcommand{\eequiv}{~{}\equiv{}~}
\newcommand{\pplus}{~{}+{}~}
\newcommand{\ccdot}{~{}\cdot{}~}
\newcommand{\llongrightarrow}{~{}\longrightarrow{}~}
\newcommand{\qlongrightarrow}{\quad{}\longrightarrow{}\quad}
\newcommand{\qqlongrightarrow}{\qquad{}\longrightarrow{}\qquad}
\newcommand{\mmid}{~{}\mid{}~}
\newcommand{\qmid}{\quad{}|{}\quad}
\newcommand{\tto}{~{}\to{}~}
\newcommand{\uuplus}{\,{}\uplus{}\,}
\newcommand{\nneq}{~{}\neq{}~}
\newcommand{\qeq}{\quad{}={}\quad}
\newcommand{\qqeq}{\qquad{}={}\qquad}
\newcommand{\lleq}{~{}\leq{}~}
\newcommand{\LL}{~{}<{}~}
\newcommand{\GG}{~{}>{}~}
\newcommand{\ggeq}{~{}\geq{}~}
\newcommand{\ssqsubseteq}{~{}\sqsubseteq{}~}
\newcommand{\iimplies}{~{}\implies{}~}
\newcommand{\mmodels}{~{}\models{}~}
\newcommand{\nnotmodels}{~{}\not\models{}~}
\newcommand{\iin}{~{}\in{}~}
\newcommand{\nnotin}{~{}\not\in{}~}
\newcommand{\wwedge}{~{}\wedge{}~}
\newcommand{\vvee}{~{}\vee{}~}

\newcommand{\cwedge}{\,{}\wedge{}\,}

%Colorful equation
% Commands for Highlighting text -- non tikz method
%\newcommand{\highlight}[2]{\colorbox{#1!17}{$\displaystyle #2$}}
%\newcommand{\highlight}[2]{\colorbox{#1!17}{$#2$}}

% Commands for Highlighting text -- non tikz method
%\renewcommand{\highlight}[2]{\colorbox{#1!17}{#2}}



%for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother

==> tikzkey.tex <==
\RequirePackage{tikz}
\RequirePackage{pgfplots}
%\usetikzlibrary{patterns}
\usetikzlibrary {arrows.meta}
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}

\usetikzlibrary{
	cd,
	math,
	decorations.markings,
	decorations.pathreplacing,
	positioning,
	arrows.meta,
	circuits.logic.US,
	shapes,
	calc,
	fit,
	quotes,
  scopes,
  patterns,
  backgrounds}

\usepgfplotslibrary{groupplots, fillbetween}


\tikzset{
        oriented WD/.style={%everything after equals replaces "oriented WD" in key.
           %every to/.style={out=0,in=180,draw},
           label/.style={
              font=\everymath\expandafter{\the\everymath\scriptstyle},
              inner sep=0pt,
              node distance=2pt and -2pt},
           semithick,
           node distance=1 and 1,
           decoration={markings, mark=at position \stringdecpos with \stringdec},
           ar/.style={postaction={decorate}},
           execute at begin picture={\tikzset{
              x=\bbx, y=\bby,
              every fit/.style={inner xsep=\bbx, inner ysep=\bby}}}
           },
        string decoration/.store in=\stringdec,
        string decoration={\arrow{stealth};},
        string decoration pos/.store in=\stringdecpos,
        string decoration pos=.7,
        bbx/.store in=\bbx,
        bbx = 1.5cm,
        bby/.store in=\bby,
        bby = 1.5ex,
        bb port sep/.store in=\bbportsep,
        bb port sep=1.5,
        % bb wire sep/.store in=\bbwiresep,
        % bb wire sep=1.75ex,
        bb port length/.store in=\bbportlen,
        bb port length=4pt,
        bb penetrate/.store in=\bbpenetrate,
        bb penetrate=0,
        bb min width/.store in=\bbminwidth,
        bb min width=1cm,
        bb rounded corners/.store in=\bbcorners,
        bb rounded corners=2pt,
        bb small/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, 
   bby=.7ex},
            bb medium/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, 
   bby=.9ex},
        bb/.code 2 args={%When you see this key, run the code below:
           \pgfmathsetlengthmacro{\bbheight}{\bbportsep * (max(#1,#2)+1) * \bby}
           \pgfkeysalso{draw,minimum height=\bbheight,minimum width=\bbminwidth,outer 
   sep=0pt,
              rounded corners=\bbcorners,thick,
              prefix after command={\pgfextra{\let\fixname\tikzlastnode}},
              append after command={\pgfextra{\draw
                 \ifnum #1=0{} \else foreach \i in {1,...,#1} {
%                    ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(-\bbportlen,0) coordinate (\fixname_in\i) -- +(\bbpenetrate,0) coordinate (\fixname_in\i')}\fi 
                    ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(0,0) coordinate (\fixname_in\i) -- +(\bbpenetrate,0) coordinate (\fixname_in\i')}\fi 
     %Define the endpoints of tickmarks
                 \ifnum #2=0{} \else foreach \i in {1,...,#2} {
%                    ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbpenetrate,0) coordinate (\fixname_out\i') -- +(\bbportlen,0) coordinate (\fixname_out\i)}\fi;
                    ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbpenetrate,0) coordinate (\fixname_out\i') -- +(0,0) coordinate (\fixname_out\i)}\fi;
              }}}
        },
        bb name/.style={append after command={\pgfextra{\node[anchor=north] at 
   (\fixname.north) {#1};}}}     
}

\pgfplotsset{
  Axis Set/.style = {
    axis lines=middle,
		every axis y label/.style={
			at={(ticklabel* cs:1)},
			anchor=south,
		},
		%			footnotesize,
		width = 6.5cm, %% As big as this example can be without spilling over onto the next slide
		height = 4cm, %% ditto
		%			ticks = none,
		xtick = {1,2,3,4},
    %ytick = {1,2,3,4,5},
    xmin = 0, 
    ymin = 0
  }
}
